Sparse Mixture-of-Experts are Domain Generalizable Learners

Human visual perception can easily generalize to out-of-distributed visual data, which is far beyond the capability of modern machine learning models. Domain generalization (DG) aims to close this gap, with existing DG methods mainly focusing on the loss function design. In this paper, we propose to explore an orthogonal direction, i.e., the design of the backbone architecture. It is motivated by an empirical finding that transformer-based models trained with empirical risk minimization (ERM) outperform CNN-based models employing state-of-the-art (SOTA) DG algorithms on multiple DG datasets. We develop a formal framework to characterize a network's robustness to distribution shifts by studying its architecture's alignment with the correlations in the dataset. This analysis guides us to propose a novel DG model built upon vision transformers, namely Generalizable Mixture-of-Experts (GMoE). Extensive experiments on DomainBed demonstrate that GMoE trained with ERM outperforms SOTA DG baselines by a large margin. Moreover, GMoE is complementary to existing DG methods and its performance is substantially improved when trained with DG algorithms.

==> archived/method.tex <==
\subsection{Visual Attributes, Conditional Sentences, and Mixture of Experts}\label{sec:method}
In this section, we discuss the connections between attributes, conditional sentences and mixture of experts. More often than not, the labels of real-world image data depend on multiple attributes. We take Caltech-UCSD Birds 200 (CUB-200) as an example~\cite{wah2011caltech}. CUB-200 includes 6,033 annotated images of birds, belonging to 200 bird species. The label is jointly determined by 25 attributes, including color (e.g., crown color), shape (e.g., wing shape), and pattern/texture (e.g., breast pattern). In a broader sense, we usually use multiple attributes to define an object. For example, the definition of an \emph{elephant} in Oxford dictionary is \emph{a very large animal with thick grey skin, large ears, two curved outer teeth called tusks and a long nose called a trunk}. The definition involves two shape attributes (i.e., large ears, two curved outer teeth, and a long nose) and one texture attribute (i.e., thick grey skin). Without multiple attributes, we cannot accurately define an elephant (e.g., both the elephants and rhinos have thick grey skin).

To detect these attributes, different filters should be applied to different patches. From an algorithmic perspective, the conditional sentences are needed


Although above intuition seems to be high-level, Sparse MoE indeed operates in this way. Please refer to Section and Appendix for details. 

% % Sparsely activated Mixture-of-Experts (Sparse MoE) model can substantially scale up the model capacity while keeping training and inference computational overhead roughly constant. 
% Through our analysis in Sec.~\ref{}, we addressed that attention mechanism could enable model better capture invariant correlation than spurious correlation. Then we addressed MoE could better align with conditional sentences and specialize to cluster-center features (\eg visual attributes).  In this section, we start with introducing generalizing to multiple domain data via learning visual attributes in Sec~\ref{method:visual-attr}. In Sec.~\ref{method:moe}, we introduce the essential components in our Sparse MoE model. Next, in Sec.~\ref{method:adapt}, we introduce main difficulties in Sparse MoE in domain generalization task and provide our key techniques to resolve these challenges. 

% % the key components of Sparse MoE architecture (in Sec.~\ref{method:moe}). Aligning with our theoretical analysis, we analyze the role of different components and how they interact with each other to make the whole architecture better perform on Domain Generalization task (in Sec.~\ref{method:module}).

% \subsection{Learning with Visual Attributes}
% \label{method:visual-attr}
% {\color {red} Due to space limitation, it might not be necessary to introduce ViT. It might be good to first introduce visual attributes/sub-cluster, then MoE structure and theoretical analysis.}

% \subsection{Essential Components in Sparse MoE}
% \label{method:moe}
% Sparse MoE is built on Vision Transformer with basic building blocks. Each block contains two essential components, the multi-head attention (MHA) layer and the mixture-of-experts (MoE) layer. The two type of layers in one block are constructed with the shortcut connection and the layer normalization. 

% Multi-head attention layer could be viewed as an ensemble of single-head attention~\cite{DBLP:journals/corr/abs-2106-09650,DBLP:conf/nips/MichelLN19}. In detail, we regard the projection weight matrix $W_o$ into $h$ parts by rows, hence $W_{o} = [W_{o_1}^{T}; \ldots; W_{o_h}^{T}]^{T}$. Given a sequence of patches $\textbf{x} = [x_1, \ldots, x_n] \in \mathbb{R}^{d}$ processed by patch-embedding layer, and a query vector $q \in \mathbb{R}^{d}$. One multi-head attention layer is parameterized by weight matrices $W_{Q}, W_{K}, W_{V} \in \mathbb{R}^{d \times d}$, the $h$ independently heads could be computed in parallel to obtain the final results:
% \begin{equation}
%     f_{\text{MHA}} (\textbf{x}, q) = \sum\limits_{i = 1}^{h} W_{o_i} \sum\limits_{j=1}^{n} \text{SoftMax}(\frac{q^{T} W_{q_i}^{T} W_{k_i} x_i}{\sqrt{d}}) W_{v_i} x_i.
% \end{equation}

% % \bli{More words on MHA layer}

% Mixture-of-experts layer contains many expert networks with a shared gating function that routes each individual patch $x_i \in \mathbf{x}$ to few experts among all the candidates. 
% We denote the multiple independent $N$ experts as $E_i, i = 1, \ldots, N$, each with specific learnable weights and not shared within the layer. Following the architecture in~\cite{DBLP:conf/nips/RiquelmePMNJPKH21}, we use multiple FFNs as experts, denoted as $E_i(\mathbf{x}) = W^{2} \phi(W^{1} \mathbf{x} ) $, where $W^{1, 2}$ are parameters of two layers MLP in each expert, and $\phi(\cdot)$ is the non-linear activation function defined as $G(\mathbf{x}) = \text{TOP}_{k}(\text{SoftMax}(\mathbf{W} \mathbf{x} + \epsilon))$, where $\text{TOP}_{k}$ operation is a one-hot embedding that sets all other elements in the output vector to zero except for the elements with the largest $k$ values (we choose $k=2$ in our scenario), and an independent noise is sampled from $\epsilon \sim \mathcal{N}(0, 1 / E^{2})$. In detail, a MoE layer is defined
% \begin{equation}
% \label{eq:moe}
%     f_{\textsc{MoE}}(\mathbf{x}) = \sum\limits^{E}_{k=1} G(\mathbf{x}) \cdot E_{i}(\mathbf{x}) =\sum\limits^{E}_{k=1} \text{TOP}_{k} (\text{SoftMax} (\mathbf{W} \mathbf{x} + \epsilon)) \cdot W^{2} \phi(W^{1} \mathbf{x} )
% \end{equation}

% \subsection{Adapting Sparse MoE to Domain Generalization}
% \label{method:adapt}
% Ideally, a successful Sparse MoE model needs to ensure the routing function $g$ gradually specialize to cluster-center features (\eg visual attributes) and divide complex problems into smaller easy-to-conquer sub-problems. However, achieving this result is difficult since finding such a gating function is highly non-convex. In this section, we will list the main difficulties on adapting MoE model to DG task and provide our key techniques.


% In Sec.~\ref{method:visual-attr}, we analyze that how to generalize to cross domain data by learning visual attributes. Then in Sec.~\ref{method:moe}, we introduce the essential components in MoE model. 

% and mixture-of-experts play an important role in domain generalization. 

% both multi-head attention and mixture-of-experts layers play an important role in a Sparse MoE model. 

% a successful Sparse MoE model needs to ensure the routing function $g$ gradually specialize to cluster-center features (\eg visual attributes) and divide complex problems into smaller easy-to-conquer sub-problems. However, achieving this result is difficult since finding such a gating function is highly non-convex. In this section, we will introduce the main difficulties on adapting MoE model to DG task and provide our key techniques.

% Motivated by~\cite{}, 

% However, to avoid imbalance issue, $g$ is usually initialized with random noise $\mathcal{N}(0, \sigma^{2})$. This would make $g$ just evenly dispatch data into each expert at the first few updates. How could ensure the routing function learn to dispatch according to cluster-center features and divide complex problems into smaller easy-to-solve one? We have the following observations:

% the MoE model may potentially degrade to singleton ViT. This imbalance issue would cause a few experts trained more rapidly than others. 
% In detail, we denote the multiple independent $N$ experts as $E_i, i = 1, \ldots, N$, each with specific learnable weights and not shared within the layer. Following the architecture in~\cite{DBLP:conf/nips/RiquelmePMNJPKH21}, we use multiple FFNs as experts, denoted as $E_i(x) = f_{\text{FFN}_i}(x) = \phi(x W^{1}) W^{2}$, where $W^{1, 2}$ are parameters of two layers MLP in each expert, and $\phi(\cdot)$ is the non-linear activation function. We use a gating network to route each token from the previous block's output to different experts. The MoE layer is denoted as 
% \begin{equation}
%     f_{\text{MoE}}(x) = \sum\limits^{N}_{i} G(x)_i f_{\text{FFN}_i}(x),
% \end{equation}
% where $x \in \mathbb{R}^{d}$ is the input to the FFN layer $f_{\text{FFN}_i}: \mathbb{R}^{d} \rightarrow \mathbb{R}^{d}$, and $G: \mathbb{R}^{d} \rightarrow \mathbb{R}^{N}$ is the routing function, which prescribes the input-conditioned weight for the experts, \eg $G(x)_i$ denotes the probability of selecting experts $E_i$ for $x$.

% Routing function is specifically defined as $G(x_i) = \text{TOP}_{k}(\text{SoftMax}(\mathbf{W}x_i + \epsilon))$, where $\text{TOP}_{k}$ operation is a one-hot embedding that sets all other elements in the output vector to zero except for the elements with the largest $k$ values (we choose $k=2$ in our scenario), and $\epsilon$ is sampled from $e \sim \mathcal{N}(0, 1 / N^{2})$. Due to space limit, we leave more details in appendix.
% Recent study shows that sub-layers in multi-head attention and FFN layers have the inherent ensemble sub-structure~\cite{DBLP:journals/corr/abs-2106-09650,DBLP:conf/nips/MichelLN19}. The sub-structure in each layer can be viewed as an ensemble of smaller sparse models. 

% then highlight the drawbacks that standard multi-head attention module usually produces redundant attention heads. 

% In this section, we introduce the working mechanism and the key component of SF-MoE architecture.
% We start with the ViT model (in Sec.~\ref{method:vit}) and highlight a drawback that standard multi-head attention usually produce redundant attention heads. Therefore, we propose SF-MoE, where sparse blocks (in Sec.~\ref{method:sparse_block}) encourage attention heads to focus on more diverse features within layers, and fusion blocks (in Sec.~\ref{method:fusion_block}) encourage the integration of diverse attentions among heads. SF-MoE can further utilize convolutional features for enhanced performance (in Sec.~\ref{method:hybrid}).

% \subsection{Preliminary: ViT and Multi-Head Attention}
% \label{method:vit}
% SF-MoE is built on Vision Transformer, which contains two essential components, the multi-head attention (MHA) layer and the feed-forward-network (FFN) layer. Each layer is constructed with the shortcut connection and the layer normalization. Recent study shows that sub-layers in multi-head attention and FFN layers have the inherent ensemble sub-structure~\cite{DBLP:journals/corr/abs-2106-09650,DBLP:conf/nips/MichelLN19}. The sub-structure in each layer can be viewed as an ensemble of smaller sparse models. In detail, we regard the projection weight matrix $W_o$ into $h$ parts by rows, hence $W_{o} = [W_{o_1}^{T}; \ldots; W_{o_h}^{T}]^{T}$. Given a sequence of patches $\textbf{x} = [x_1, \ldots, x_n] \in \mathbb{R}^{d}$ processed by patch-embedding layer, and a query vector $q \in \mathbb{R}^{d}$. One multi-head attention layer is parameterized by weight matrices $W_{Q}, W_{K}, W_{V} \in \mathbb{R}^{d \times d}$, the $h$ independently heads could be computed in parallel to obtain the final results: 
% \begin{equation}
%     f_{\text{MHA}} (\textbf{x}, q) = \sum\limits_{i = 1}^{h} W_{o_i} \sum\limits_{j=1}^{n} \text{SoftMax}(\frac{q^{T} W_{q_i}^{T} W_{k_i} x_i}{\sqrt{d}}) W_{v_i} x_i.
% \end{equation}

% \begin{figure}[t]
%      \centering
%      \includegraphics[width=0.95\textwidth]{figures/bird_vis.pdf}
%      \caption{Comparison between multi-head attention visualization on the last block of vanilla ViT and SF-MoE. Images are selected from \textit{Real} domain in DomainNet.}
%      \label{fig:3}
% \end{figure}

% \subsection{Sparse Blocks: Disentangling Attentions}
% \label{method:sparse_block}
% To avoid head redundancy and improve network sparsity, we introduce a mixture-of-experts (MoE) layer after the multi-head attention (MHA) layer and name it the sparse block. 
% Next, we study the innate disentanglement and sparsity mechanism in a sparse block.

% \begin{figure}[tp]
%      \centering
%      \includegraphics[width=\textwidth]{figures/arch_comp.png}
%      \caption{Different compositions of sparse/fusion blocks in a $12$-block ViT. We denote sparse/fusion blocks with $\mathbf{S}$ and $\mathbf{F}$, respectively. $[\mathbf{S}, \mathbf{F}] \times 6$ means alternating sparse/fusion blocks from shallow to deep for 6 times. \textbf{Left}: Out-of-domain accuracy in different iterations during training on \textit{Real} domain from DomainNet. \textbf{Right}: Overall accuracy (average on every domain) in VLCS, PACS and OfficeHome.}
%      \label{fig:4}
% \end{figure}

% \subsection{Fusion Blocks: Aggregating Attentions}
% \label{method:fusion_block}
% In sparse block, the MoE layer leverages a routing network to learn patch-to-expert affinity. 
% % The learned routing network should, in theory, allow identical or relevant patches to be sent to the same expert. Ideally, when all patches are invariant to the routing network, a sub-optimal strategy would result in that a few experts accommodate most of patches and leave rest of the experts underparametrized.
% In theory, the learned routing network should allocate identical or related patches to the same expert. Ideally, when all patches are invariant to the routing network, a suboptimal strategy would result in a few experts adapting most of the patches, while the remaining experts are under-parameterized.
% Under-parametrization may induce a large auxiliary loss for load balancing, but less effective routing.
% This will make training more challenging, since more experts in different layers would require more training data that is properly balanced to each expert~\cite{DBLP:conf/icml/LewisBDGZ21}.

% Empirically, in Figure~\ref{fig:4}, we find that keep adding sparse blocks (\eg $[\mathbf{S}] \times 12$) would result in performance drop. We opine that increasing sparsity also results in retaining more spurious information. More spurious information will falsify the network to capture spurious correlation in training data, and also weaken the generalization performance.

% Due to the aforementioned difficulties, we cannot directly apply V-MoE~\cite{DBLP:conf/nips/RiquelmePMNJPKH21} structure with a full sparse blocks pattern. To alleviate this issue, we propose a fusion block with a MHA layer and a dense FFN layer $f_{\text{dense}}(x) = \phi(xW^{1}) W^{2}, W^{1} \in \mathbb{R}^{d \times k}, W^{2} \in \mathbb{R}^{k \times d}$. Empirically, we set $k=4d$. The dense FFN layer integrates and transforms diverse attentions among different heads. Accordingly, our empirical investigation in Figure~\ref{fig:4} indicates that balancing the number of sparse/fusion blocks (\eg 6 sparse blocks, 6 fusion blocks in 12-block ViT) would improve out-of-domain generalization performance in three datasets.

% \subsection{Hybrid SF-MoE: Integrating Convolutional Features}
% \label{method:hybrid}
% The primary elements of multi-head attention and sparse/fusion blocks are MLPs, which could improve the utilization of information while also increase the computational cost. 
% A natural variation~\cite{DBLP:conf/iclr/DosovitskiyB0WZ21} is proposed to combine CNN~\cite{DBLP:journals/neco/LeCunBDHHHJ89} into Transformer architecture. We adopt this design and introduce ResNet~\cite{he2016deep} backbone for patch embedding. ResNet patch embedding layer would extract a feature map which is much smaller than original $16 \times 16$ patch embedding, and still preserves local information~\cite{DBLP:conf/iclr/IslamJB20}. 
% This property brings a positive impact on DG task since images contain redundant information between pixels in natural images.
% % Positional information hence expedite subsequent multi-head attention layers and sparse/fusion blocks. 

% We adopt the HybridViT pretrained on ImageNet-21k and fine-tuned on ImageNet-1k, then replace basic blocks of HybridViT with sparse/fusion blocks. To make fair comparison, we compare Hybrid SF-MoE with other counterparts that also pretrained on ImageNet-21k dataset. Hybrid SF-MoE, as an efficient variant of SF-MoE, could improve performance on large-scale datasets with the lowest run-time memory and throughput time.

==> archived/related_work.tex <==
\section{Related Works}
In this section, we discuss the most relevant works in the following topics.
% {\color {red} We'd better make this section short to leave space for the main text}

\subsection{Domain Generalization}
Domain Generalization (DG) aims to keep the high performance of the machine learning models even on the domains that are different from the training (source) domain.
The following are the main categories of mainstream domain generalization research. 

\textbf{(1) Domain Alignment}: Aligning domain distributions and finding invariance between domains has been often studied with empirical results and theoretical proofs~\cite{DBLP:journals/jmlr/GaninUAGLLML16,DBLP:conf/nips/HoffmanMZ18}. Specifically, researchers seek explicitly aligning feature distributions based on the maximum mean discrepancy (MMD)~\citep{DBLP:journals/tnn/PanTKY11,DBLP:journals/corr/TzengHZSD14,DBLP:conf/mm/WangFCYHY18}, or second order correlation~\citep{DBLP:conf/aaai/SunFS16,DBLP:conf/eccv/SunS16,DBLP:conf/wacv/PengS18}, moment matching~\citep{DBLP:conf/iccv/PengBXHSW19} and Wasserstein distance~\citep{DBLP:journals/corr/abs-2007-10573,lyu2021barycentric}, etc.
Besides aligning distributions in feature space, Arjovsky et al.~\cite{DBLP:journals/corr/abs-1907-02893} propose IRM to learn an ideal invariant classifier on top of the representation space. However, Rosenfeld et al.~\cite{DBLP:conf/iclr/RosenfeldRR21} claims that IRM need at least $d_s$ environments to learn optimal invariant predictors where $d_s$ is the dimension of spurious features. Similar effect has also been discussed in other recent works~\cite{DBLP:conf/aistats/KamathTSS21,DBLP:conf/icml/KruegerCJ0BZPC21} and many improvements~\cite{DBLP:conf/iclr/RosenfeldRR21,DBLP:conf/nips/AhujaCZGBMR21,DBLP:journals/corr/abs-2106-06333} have been studied.

\textbf{(2) Data Manipulation}: Diverse training data are intuitively helpful for improving generalization, researchers proposed manipulation/augmentation techniques ~\cite{DBLP:conf/eccv/NazariK20,DBLP:conf/iclr/RiemerCALRTT19}, domain randomization~\cite{DBLP:journals/corr/abs-1807-09834,DBLP:conf/iccv/YueZZSKG19,DBLP:conf/iccv/ZakharovKI19}. Furthermore, some methods~\cite{DBLP:conf/iclr/RiemerCALRTT19,DBLP:conf/cvpr/QiaoZP20,DBLP:conf/nips/LiuLYW18,DBLP:journals/corr/abs-2002-12169,DBLP:conf/nips/ZhaoLYG0HCK19,DBLP:conf/aaai/ZhaoWLWGXDK21,DBLP:journals/ijcv/ZhaoLXYDK21} exploit generated data samples to enhance the model generalization ability. 

\textbf{(3) Ensemble Learning} methods~\cite{DBLP:conf/icip/ManciniBC018,DBLP:journals/corr/abs-2011-12672} assume the overall prediction should be inferred by a combination of the different models.
Zhou et al.~\cite{DBLP:journals/tip/ZhouYQX21} proposed a shared CNN feature extractor as backbone with domain-specific classifiers, each of which is an expert in its own domain but a non-expert in others.
SWAD~\cite{cha2021swad} inhibits models from being overfit to local sharp minima by averaging model weights below a validation loss threshold. By averaging the model weights from beginning to end, EoA~\cite{DBLP:journals/corr/abs-2110-10832} further reduces the amount of computations on the validation set. SEDGE~\cite{DBLP:journals/corr/abs-2203-04600} leverages multiple pretrained models and selects best fit combination weights per sample to reach better accuracy with less trainable parameters and training time.

\subsection{Algorithmic Alignment}
The algorithmic alignment framework~\cite{xu2019what} was originally proposed for understanding the effectiveness of specialized network structures in reasoning tasks. Specifically, it characterizes the generalization bound of reasoning tasks by studying the alignment between the reasoning algorithm and the computation graph of the neural network. The underlying intuition is that if they align well, the neural network only needs to learn \emph{simple} functions, which leads to better sample efficiency. This framework was further extended in \cite{li2021does} to investigate the impact of neural architecture in the robustness to noisy labels. This paper is the first attempt to understand domain generalization via algorithmic alignment, which provides a orthogonal direction to existing works.

\subsection{Vision Transformers}
Originated from the machine translation tasks, Transformer~\cite{DBLP:conf/nips/VaswaniSPUJGKP17} has received great attention in computer vision~\cite{DBLP:conf/iclr/DosovitskiyB0WZ21,DBLP:conf/iccv/LiuL00W0LG21,wang2022image} for their unprecedented performance in image recognition, semantic segmentation, and visual question answering. In addition to strong performance, some recently works empirically demonstrate the robustness of the ViTs over CNNs in terms of adversarial noise~\cite{DBLP:journals/corr/abs-2110-07858} and distribution shift~\cite{zhang2022delving}. In this paper, we obtain a theoretical understanding of robustness of ViT-based models from the algorithmic alignment perspective. The analysis also motivates us to employ mixture-of-experts to enhance the performance of ViT models. 

\subsection{Sparse Mixture-of-Experts}
Mixture-of-Experts models, or MoEs, make use of the outputs from several sub-models (experts) through an input-dependent routing mechanism for stronger model performance~\cite{DBLP:journals/neco/JacobsJNH91,DBLP:journals/neco/JordanJ94}. 
This training paradigm has led to the development of a plethora of methods for a wide ranges of applications~\cite{hu1997patient,tani1999learning}. However, in the era of bigs models, will inevitably introduce even larger model size and longer inference time. Sparse MoEs~\cite{DBLP:conf/iclr/ShazeerMMDLHD17} was proposed with their routers to select only a few of experts, so that the inference time is on-par with the standalone counterpart. As a result, sparse MoEs are promising approaches to scale up vision models~\cite{DBLP:conf/nips/RiquelmePMNJPKH21}. In this paper, we prove that Sparse MoEs algorithmically align conditional sentences, which demonstrate the unique advantage of Sparse MoEs in DG. In addition, we discuss the bag of tricks to adapt the original Sparse MoEs to DG setting.

\subsection{Neural Architecture Design in DG}
There have been some attempts on neural architecture search for domain generalization~\cite{DBLP:conf/icml/ZhangAX0C21,bai2021ood}. It was conjectured in~\cite{DBLP:conf/icml/ZhangAX0C21} that there exists unbiased functional subnetworks in biased models and modular risk minimization was proposed to search for such subnetworks. In~\cite{bai2021ood}, neural architecture search was employed to identify better CNN-based architectures for DG. Nevertheless, there is limited theoretical understanding of how neural architecture impacts its performance on domain generalization and this work is an initial attempt. Furthermore, we demonstrate that Sparse MoE models are domain generalizable learners, which is orthogonal to substructure search~\cite{DBLP:conf/icml/ZhangAX0C21} and NAS of CNNs-based models~\cite{bai2021ood}.

% \subsection{Vision Transformer}
% Originated from the machine translation tasks, Transformer~\cite{DBLP:conf/nips/VaswaniSPUJGKP17} has received great attention from broader research communities beyond natural language processing~\cite{han2022survey,DBLP:conf/iclr/HuangVUSHSDHDE19,irwin2022chemformer,shih2022theme,DBLP:conf/emnlp/WolfDSCDMCRLFDS20}.
% ViT~\cite{DBLP:conf/iclr/DosovitskiyB0WZ21} is marked as the first successful attempt on implementing transformer model into computer vision tasks, which simply splits the whole image into patches and feeds them into Transformer encoders with multi-head attention mechanisms.
% Since then, many Transformer variants, such as Swin Transformer~\cite{DBLP:conf/iccv/LiuL00W0LG21}, MViT~\cite{DBLP:conf/iccv/0001XMLYMF21}, PVT~\cite{DBLP:conf/iccv/WangX0FSLL0021}, and PiT~\cite{DBLP:conf/iccv/HeoYHCCO21}, have been presented by introducing hierarchical~\cite{DBLP:journals/pami/KrugerJKLLPRW13} and shift-invariant~\cite{DBLP:conf/cvpr/KayhanG20} priors that are proved being useful to vision tasks by classic CNNs~\cite{he2016deep,DBLP:conf/nips/KrizhevskySH12}.
% Despite all these great improvement on vision transformer structures, in this paper, we develop our SF-MoE model based on the most classic and extensible ViT model.
% Besides, some existing works explore and conclude the robustness of the attention-based ViTs over CNNs~\cite{DBLP:journals/corr/abs-2105-07581,DBLP:conf/iccv/BhojanapalliCGL21}, and attempting to improve the ViT robustness via techniques such as patch-based negative augmentation~\cite{DBLP:journals/corr/abs-2110-07858} and extra fully attentional design~\cite{DBLP:journals/corr/abs-2204-12451}. 
% To further enhance their robustness, in this paper, we explore the design of Sparse MoEs for ViT models on the domain generalization platform.

% \subsection{Sparse Mixture-of-Experts}
% % Moe
% Mixture-of-Experts models, or MoEs, make use of the outputs from several sub-models (experts) through an input-dependent routing mechanism for stronger model performance~\cite{DBLP:journals/neco/JacobsJNH91,DBLP:journals/neco/JordanJ94}. 
% This training paradigm has led to the development of a plethora of methods for a wide ranges of applications~\cite{hu1997patient,tani1999learning}, especially in natural language processing~\cite{serdyukov2008modeling,DBLP:conf/iclr/ShazeerMMDLHD17} and computer vision~\cite{gavrila2007multi,gross2017hard}
% However, multiple sub-models will inevitably introduce larger model size and longer inference time.
% To address this problem, Sparse MoEs~\cite{DBLP:conf/iclr/ShazeerMMDLHD17,DBLP:conf/nips/RiquelmePMNJPKH21,DBLP:conf/iclr/LepikhinLXCFHKS21,DBLP:journals/corr/abs-2101-03961} are proposed with their routers to select only a few of experts, so that the inference time is on-par with the standalone counterpart. 
% The sparsity mechanism finally helped the successful deployment of recently scaled language models reaching trillions of parameters~\cite{DBLP:journals/corr/abs-2204-02311,DBLP:journals/corr/abs-2101-03961}.
% Some following works attempt to dive deep to explore the merits of Sparse MoEs. As analyzed in~\cite{DBLP:journals/corr/abs-2110-03360}, Sparse MoE can be seen as a dynamic ensemble of subnetworks. This mechanism explicitly disentangles information within structures and prevents the model from absorbing easy spurious correlations~\cite{DBLP:conf/eccv/BeeryHP18}. In this work, we, for the first time, introduce Sparse MoEs into the DG community and provide several valuable insights based on the specific setting.


==> archived/theory.tex <==
\section{Theoretical Analysis}
In this section, we endeavor to provide theoretical understanding for the proposed method. Specifically, we are interested in the following questions: 1) why neural architecture is important to domain generalization; 2) when attention is better than convolution; 3) when MoE is useful in Transformer. Our analysis is based on algorithmic alignment framework. 
\subsection{Impact of Neural Architecture in Domain Generalization}




From the above discussion, we know that 


\subsection{MoE versus ViT}

\begin{wrapfigure}[22]{R}{0.30\textwidth}
    %\vspace{-2mm}
    \begin{algorithm}[H]\label{alg:condition}
      \DontPrintSemicolon
      \SetKwFunction{Grad}{Grad}
      \SetKwProg{Fn}{Function}{:}{}
      \SetKwFor{uFor}{For}{do}{}
      \SetKwFor{ForPar}{For all}{do in parallel}{}
      \SetKwFunction{ADMMucell}{ADMMu-cell}
      \SetKwFunction{ADMMu}{ADMMu}
      Define $A_i \subset \mathbb{R}, i = 1, \cdots, M$\;
      \Switch(){$h_1(\bm{x})$}
      { \Case{$A_i$}{apply $h_{i+1}$ to $\bm{x}$}}
    \caption{\texttt{Conditional sentences} }\label{algo:admmu}
    \end{algorithm}
\end{wrapfigure} 
\begin{lemma} MoE module with $N \geq M$ experts well aligns the conditional sentences in Algorithm \ref{alg:condition}. 
\end{lemma}
\begin{proof}
We define the mapping $H(x) = [1_{A_1}, \cdots, 1_{A_M}] \in \mathbb{R}^M$, where $1_{A_i}$ is the indicator function on interval $A_i$. To show the alignment between MoE and conditional sentences, we define the module functions $f_1, \cdots, f_{N}$ and neural network modules $\mathcal{N}_1, \cdots, \mathcal{N}_{N}$ as
\begin{align*}
    f_i = \left\{
\begin{aligned}
&H \circ h_1, &&\text{if } i=1,  \\
&h_{((i-2)\text{mod} M)+2}, && \text{o.w.},
\end{aligned}
\right. \quad \mathcal{N}_i = \left\{
\begin{aligned}
&G, &&\text{if }i=1,  \\
&f_{\text{FFN}_i}, && \text{o.w.},
\end{aligned}
\right.
\end{align*}
MoE well aligns the conditional sentences as replace $\mathcal{N}_i$ with $f_i$, MoE network simulates Algorithm \ref{alg:condition}.
\end{proof}











==> archived/theory_backup.tex <==
\begin{definition} (OOD Learnability) Fix an error parameter $\epsilon>0$ and a failure probability $\delta \in (0,1)$. Suppose training samples $\{(\bm{x}_i^{(1)},\bm{y}_i^{(1)})\}_{i=1}^M$ are i.i.d. samples from distribution $D_{tr}$. Each test sample $(\bm{x}^{(te)},\bm{y}^{(te)})$ is drawn from distribution $D_{te}$ and satisfies $\bm{y} = g(\bm{x})$. Let $f = \mathcal{A}(\{\bm{x}_i,\bm{y}_i\}_{i=1}^M)$ be the function generated by a learning algorithm $\mathcal{A}$. Then $g$ is $(M,\epsilon,\delta,\mathcal{D}_1,\mathcal{D}_2)$-learnable with $\mathcal{A}$ if 
\begin{align*}
    \mathbb{P}_{\bm{x} \sim \mathcal{D}_2}[\|f(\bm{x}) - g(\bm{x})\| \leq \epsilon] \geq 1 - \delta
\end{align*}
The sample complexity $\mathcal{C}_{\mathcal{A}}$ is the minimum $M$ such that $g$ is $(M,\epsilon,\delta,\mathcal{D}_1,\mathcal{D}_2)$-learnable with $\mathcal{A}$.
\end{definition}

\paragraph{Label generation model of image recognition:} In image recognition, the label is always given by human beings. To recognize an image, a human will first disentangle it into several compact and semantic concepts, and then xxx. Thus, our label generation model is given by
\begin{align}\label{eq:label_gen}
    \bm{x} \xrightarrow{v_1(\bm{x})} (\bm{z}_c,\bm{z}_e) \xrightarrow{v_2(\bm{z}_c)} \bm{y}
\end{align}
where $\bm{z}_c$ is the feature that leads human predicting the label and follows the same distribution across all domains. The target function we should learn is $g = v_1 \circ v_2$.

\paragraph{Difficulty for OOD generalization:} Compared with IID generalization in classic machine learning, a unique difficulty of OOD generalization is that they may overfit to the training distribution. This is because two different functions can have the same restriction on training data distribution, which is a low-dimensional manifold. We formalize this concept in the following.  
\begin{definition} (Overfit to Training Distribution) A learning algorithm $f = \mathcal{A}(\{\bm{x}_i,\bm{y}_i\}_{i=1}^M)$ is said to overfit to training distribution if $g$ is $(M,\epsilon,\delta,\mathcal{D}_1,\mathcal{D}_1)$-learnable with $\mathcal{A}$, but not $(M,\epsilon,\delta,\mathcal{D}_1,\mathcal{D}_2)$-learnable with $\mathcal{A}$.
\end{definition}

\subsection{Formalization of Alignment}
\begin{definition} (Algorithmic Alignment) Let $\mathcal{N}$ denote a neural network with 
    
\end{definition}

\begin{theorem} (Informal; Better Alignment Implies Better IID Generalization) Fix $\epsilon$ and $\delta$

\end{theorem}



\subsection{Better Alignment Implies Better Domain Generalization}
\begin{assumption} (Low-level Disentanglement) For each test sample $\bm{x}$, suppose we can decompose the low-level features as $[\bm{z}_c, \bm{z}_e] = \mathcal{N}_1(\bm{x})$. A feature belongs to $\bm{z}_c$ if it is a in-distribution feature of training datasets other wises it belongs to $\bm{z}_e$.
\end{assumption}

\begin{assumption} (Invariant Relation) Assume there exists a function $g_1$ such that for each training training distribution $D \in \mathcal{D}_{tr} \cup \{D_{te}\}$ we have $\mathbb{P}_{D}[\|g_1(\mathcal{N}_c(\bm{x})) - g(\bm{x})\| \leq \epsilon] > 1 - \delta$.
\end{assumption}

\begin{assumption} (Spurious Correlation) Assume there exists a function $g_2$ such that for each training training distribution $D \in \mathcal{D}_{tr}$ we have $\mathbb{P}_{D}[\|g_2(\mathcal{N}_c(\bm{x})) - g(\bm{x})\| \leq \epsilon] > 1 - \delta$ and for test distribution we have $\mathbb{P}_{D_{te}}[\|g_2(\mathcal{N}_c(\bm{x})) - g(\bm{x})\| > \epsilon] > 1 - \delta$.
\end{assumption}
\begin{remark} (Uncontrolled generalization of $\bm{z}_e$ with nonlinear function approximation) If the feature is out of distribution for any training domain, it may hurt or help generalization . 

\end{remark}
\begin{theorem} (Impact of architecture for domain generalization) 
\begin{itemize}
    \item (Good architecture succeed in generalization) If the pretrained neural network $\mathcal{N}$ well-aligned with $g_1$, then we have 
    \begin{align*}
        \mathbb{P}_{D}[\|\mathcal{N}(\bm{x}) - g(\bm{x})\| \leq O(\epsilon)] > 1 - O(\delta)
    \end{align*}
    \item (Bad architecture fail in generalization)
\end{itemize}

\end{theorem}


